Domination and Cut Problems on Chordal Graphs with Bounded Leafage

The leafage of a chordal graph G is the minimum integer l such that G can be realized as an intersection graph of subtrees of a tree with l leaves. We consider structural parameterization by the leafage of classical domination and cut problems on chordal graphs. Fomin, Golovach, and Raymond [ESA 2018, Algorithmica 2020] proved, among other things, that Dominating Set on chordal graphs admits an algorithm running in time $2^{O(l^2)} n^{O(1)}$. We present a conceptually much simpler algorithm that runs in time $2^{O(l)} n^{O(1)}$. We extend our approach to obtain similar results for Connected Dominating Set and Steiner Tree. We then consider the two classical cut problems MultiCut with Undeletable Terminals and Multiway Cut with Undeletable Terminals. We prove that the former is W[1]-hard when parameterized by the leafage and complement this result by presenting a simple $n^{O(l)}$-time algorithm. To our surprise, we find that Multiway Cut with Undeletable Terminals on chordal graphs can be solved, in contrast, in $n^{O(1)}$-time.

==> main.bbl.tex <==
\begin{thebibliography}{10}

\bibitem{DBLP:journals/dam/Alcon14}
Liliana Alc{\'{o}}n.
\newblock On asteroidal sets in chordal graphs.
\newblock {\em Discret. Appl. Math.}, 164:482--491, 2014.
\newblock \href {https://doi.org/10.1016/j.dam.2013.04.019}
  {\path{doi:10.1016/j.dam.2013.04.019}}.

\bibitem{DBLP:journals/corr/ArvindNPZ22}
Vikraman Arvind, Roman Nedela, Ilia Ponomarenko, and Peter Zeman.
\newblock Testing isomorphism of chordal graphs of bounded leafage is
  fixed-parameter tractable.
\newblock {\em CoRR}, abs/2107.10689, 2021.
\newblock URL: \url{https://arxiv.org/abs/2107.10689}, \href
  {http://arxiv.org/abs/2107.10689} {\path{arXiv:2107.10689}}.

\bibitem{DBLP:conf/wads/BalakrishnanRR93}
Hari Balakrishnan, Anand Rajaraman, and C.~Pandu Rangan.
\newblock Connected domination and steiner set on asteroidal triple-free
  graphs.
\newblock In Frank K. H.~A. Dehne, J{\"{o}}rg{-}R{\"{u}}diger Sack, Nicola
  Santoro, and Sue Whitesides, editors, {\em Algorithms and Data Structures,
  Third Workshop, {WADS} '93, Montr{\'{e}}al, Canada, August 11-13, 1993,
  Proceedings}, volume 709 of {\em Lecture Notes in Computer Science}, pages
  131--141. Springer, 1993.
\newblock \href {https://doi.org/10.1007/3-540-57155-8\_242}
  {\path{doi:10.1007/3-540-57155-8\_242}}.

\bibitem{DBLP:journals/networks/BarnetsonBEHPR21}
Kathleen~D. Barnetson, Andrea~C. Burgess, Jessica~A. Enright, Jared Howell,
  David~A. Pike, and Brady Ryan.
\newblock The firebreak problem.
\newblock {\em Networks}, 77(3):372--382, 2021.
\newblock \href {https://doi.org/10.1002/net.21975}
  {\path{doi:10.1002/net.21975}}.

\bibitem{DBLP:journals/mst/BelmonteKLMOS21}
R{\'{e}}my Belmonte, Eun~Jung Kim, Michael Lampis, Valia Mitsou, Yota Otachi,
  and Florian Sikora.
\newblock Token sliding on split graphs.
\newblock {\em Theory Comput. Syst.}, 65(4):662--686, 2021.
\newblock \href {https://doi.org/10.1007/s00224-020-09967-8}
  {\path{doi:10.1007/s00224-020-09967-8}}.

\bibitem{DBLP:journals/algorithmica/BergougnouxPT22}
Benjamin Bergougnoux, Charis Papadopoulos, and Jan~Arne Telle.
\newblock Node multiway cut and subset feedback vertex set on graphs of bounded
  mim-width.
\newblock {\em Algorithmica}, 84(5):1385--1417, 2022.
\newblock \href {https://doi.org/10.1007/s00453-022-00936-w}
  {\path{doi:10.1007/s00453-022-00936-w}}.

\bibitem{DBLP:journals/ipl/Bertossi84}
Alan~A. Bertossi.
\newblock Dominating sets for split and bipartite graphs.
\newblock {\em Inf. Process. Lett.}, 19(1):37--40, 1984.

\bibitem{DBLP:journals/siamcomp/BousquetDT18}
Nicolas Bousquet, Jean Daligault, and St{\'{e}}phan Thomass{\'{e}}.
\newblock Multicut is {FPT}.
\newblock {\em {SIAM} J. Comput.}, 47(1):166--207, 2018.
\newblock \href {https://doi.org/10.1137/140961808}
  {\path{doi:10.1137/140961808}}.

\bibitem{DBLP:journals/dm/Buneman74}
Peter Buneman.
\newblock A characterisation of rigid circuit graphs.
\newblock {\em Discret. Math.}, 9(3):205--212, 1974.

\bibitem{DBLP:conf/soda/Cao16}
Yixin Cao.
\newblock Linear recognition of almost interval graphs.
\newblock In Robert Krauthgamer, editor, {\em Proceedings of the Twenty-Seventh
  Annual {ACM-SIAM} Symposium on Discrete Algorithms, {SODA} 2016, Arlington,
  VA, USA, January 10-12, 2016}, pages 1096--1115. {SIAM}, 2016.
\newblock \href {https://doi.org/10.1137/1.9781611974331.ch77}
  {\path{doi:10.1137/1.9781611974331.ch77}}.

\bibitem{DBLP:journals/siamcomp/Chang98}
Maw{-}Shang Chang.
\newblock Efficient algorithms for the domination problems on interval and
  circular-arc graphs.
\newblock {\em {SIAM} J. Comput.}, 27(6):1671--1694, 1998.
\newblock \href {https://doi.org/10.1137/S0097539792238431}
  {\path{doi:10.1137/S0097539792238431}}.

\bibitem{DBLP:journals/dam/ChaplickS14}
Steven Chaplick and Juraj Stacho.
\newblock The vertex leafage of chordal graphs.
\newblock {\em Discret. Appl. Math.}, 168:14--25, 2014.
\newblock \href {https://doi.org/10.1016/j.dam.2012.12.006}
  {\path{doi:10.1016/j.dam.2012.12.006}}.

\bibitem{DBLP:journals/talg/ChitnisCHM15}
Rajesh~Hemant Chitnis, Marek Cygan, Mohammad~Taghi Hajiaghayi, and D{\'{a}}niel
  Marx.
\newblock Directed subset feedback vertex set is fixed-parameter tractable.
\newblock {\em {ACM} Trans. Algorithms}, 11(4):28:1--28:28, 2015.
\newblock \href {https://doi.org/10.1145/2700209} {\path{doi:10.1145/2700209}}.

\bibitem{DBLP:journals/siamcomp/ChitnisHM13}
Rajesh~Hemant Chitnis, MohammadTaghi Hajiaghayi, and D{\'{a}}niel Marx.
\newblock Fixed-parameter tractability of directed multiway cut parameterized
  by the size of the cutset.
\newblock {\em {SIAM} J. Comput.}, 42(4):1674--1696, 2013.
\newblock \href {https://doi.org/10.1137/12086217X}
  {\path{doi:10.1137/12086217X}}.

\bibitem{DBLP:books/sp/CyganFKLMPPS15}
Marek Cygan, Fedor~V. Fomin, Lukasz Kowalik, Daniel Lokshtanov, D{\'{a}}niel
  Marx, Marcin Pilipczuk, Michal Pilipczuk, and Saket Saurabh.
\newblock {\em Parameterized Algorithms}.
\newblock Springer, 2015.
\newblock \href {https://doi.org/10.1007/978-3-319-21275-3}
  {\path{doi:10.1007/978-3-319-21275-3}}.

\bibitem{DBLP:conf/walcom/FigueiredoLMS22}
Celina M.~H. de~Figueiredo, Raul Lopes, Alexsander~Andrade de~Melo, and Ana
  Silva.
\newblock Parameterized algorithms for steiner tree and dominating set:
  Bounding the leafage by the vertex leafage.
\newblock In Petra Mutzel, Md.~Saidur Rahman, and Slamin, editors, {\em
  {WALCOM:} Algorithms and Computation - 16th International Conference and
  Workshops, {WALCOM} 2022, Jember, Indonesia, March 24-26, 2022, Proceedings},
  volume 13174 of {\em Lecture Notes in Computer Science}, pages 251--262.
  Springer, 2022.
\newblock \href {https://doi.org/10.1007/978-3-030-96731-4\_21}
  {\path{doi:10.1007/978-3-030-96731-4\_21}}.

\bibitem{DBLP:books/daglib/Diestel12}
Reinhard Diestel.
\newblock {\em Graph Theory, 4th Edition}, volume 173 of {\em Graduate texts in
  mathematics}.
\newblock Springer, 2012.

\bibitem{DBLP:journals/algorithmica/DrangeDH16}
P{\aa}l~Gr{\o}n{\aa}s Drange, Markus~S. Dregi, and Pim van~'t Hof.
\newblock On the computational complexity of vertex integrity and component
  order connectivity.
\newblock {\em Algorithmica}, 76(4):1181--1202, 2016.
\newblock \href {https://doi.org/10.1007/s00453-016-0127-x}
  {\path{doi:10.1007/s00453-016-0127-x}}.

\bibitem{DBLP:journals/algorithmica/FominGR20}
Fedor~V. Fomin, Petr~A. Golovach, and Jean{-}Florent Raymond.
\newblock On the {T}ractability of {O}ptimization {P}roblems on {H}-graphs.
\newblock {\em Algorithmica}, 82(9):2432--2473, 2020.
\newblock \href {https://doi.org/10.1007/s00453-020-00692-9}
  {\path{doi:10.1007/s00453-020-00692-9}}.

\bibitem{DBLP:journals/algorithmica/FominHKPV14}
Fedor~V. Fomin, Pinar Heggernes, Dieter Kratsch, Charis Papadopoulos, and Yngve
  Villanger.
\newblock Enumerating minimal subset feedback vertex sets.
\newblock {\em Algorithmica}, 69(1):216--231, 2014.
\newblock \href {https://doi.org/10.1007/s00453-012-9731-6}
  {\path{doi:10.1007/s00453-012-9731-6}}.

\bibitem{DBLP:conf/wg/FominKW04}
Fedor~V. Fomin, Dieter Kratsch, and Gerhard~J. Woeginger.
\newblock Exact (exponential) algorithms for the dominating set problem.
\newblock In Juraj Hromkovic, Manfred Nagl, and Bernhard Westfechtel, editors,
  {\em Graph-Theoretic Concepts in Computer Science, 30th International
  Workshop,WG 2004, Bad Honnef, Germany, June 21-23, 2004, Revised Papers},
  volume 3353 of {\em Lecture Notes in Computer Science}, pages 245--256.
  Springer, 2004.
\newblock \href {https://doi.org/10.1007/978-3-540-30559-0\_21}
  {\path{doi:10.1007/978-3-540-30559-0\_21}}.

\bibitem{ford_fulkerson}
L.~R. Ford and D.~R. Fulkerson.
\newblock Maximal flow through a network.
\newblock {\em Canadian Journal of Mathematics}, 8:399–404, 1956.
\newblock \href {https://doi.org/10.4153/CJM-1956-045-5}
  {\path{doi:10.4153/CJM-1956-045-5}}.

\bibitem{Gavril1974TheIG}
Fanica Gavril.
\newblock The intersection graphs of subtrees in tree are exactly the chordal
  graphs.
\newblock {\em Combinatorica}, 1974.

\bibitem{gilmore_hoffman_1964}
P.~C. Gilmore and A.~J. Hoffman.
\newblock A characterization of comparability graphs and of interval graphs.
\newblock {\em Canadian Journal of Mathematics}, 16:539–548, 1964.
\newblock \href {https://doi.org/10.4153/CJM-1964-055-5}
  {\path{doi:10.4153/CJM-1964-055-5}}.

\bibitem{DBLP:journals/siamdm/GolovachHHP15}
Petr~A. Golovach, Pinar Heggernes, Pim van~'t Hof, and Christophe Paul.
\newblock Hadwiger number of graphs with small chordality.
\newblock {\em {SIAM} J. Discret. Math.}, 29(3):1427--1451, 2015.
\newblock \href {https://doi.org/10.1137/140975279}
  {\path{doi:10.1137/140975279}}.

\bibitem{golumbic2004algorithmic}
Martin~Charles Golumbic.
\newblock {\em Algorithmic graph theory and perfect graphs}.
\newblock Elsevier, 2004.

\bibitem{DBLP:journals/eor/GuoHKNU08}
Jiong Guo, Falk H{\"{u}}ffner, Erhan Kenar, Rolf Niedermeier, and Johannes
  Uhlmann.
\newblock Complexity and exact algorithms for vertex multicut in interval and
  bounded treewidth graphs.
\newblock {\em Eur. J. Oper. Res.}, 186(2):542--553, 2008.
\newblock \href {https://doi.org/10.1016/j.ejor.2007.02.014}
  {\path{doi:10.1016/j.ejor.2007.02.014}}.

\bibitem{DBLP:conf/esa/HabibS09}
Michel Habib and Juraj Stacho.
\newblock Polynomial-time algorithm for the leafage of chordal graphs.
\newblock In Amos Fiat and Peter Sanders, editors, {\em Algorithms - {ESA}
  2009, 17th Annual European Symposium, Copenhagen, Denmark, September 7-9,
  2009. Proceedings}, volume 5757 of {\em Lecture Notes in Computer Science},
  pages 290--300. Springer, 2009.
\newblock \href {https://doi.org/10.1007/978-3-642-04128-0\_27}
  {\path{doi:10.1007/978-3-642-04128-0\_27}}.

\bibitem{DBLP:journals/ejc/HabibS12}
Michel Habib and Juraj Stacho.
\newblock Reduced clique graphs of chordal graphs.
\newblock {\em Eur. J. Comb.}, 33(5):712--735, 2012.
\newblock \href {https://doi.org/10.1016/j.ejc.2011.09.031}
  {\path{doi:10.1016/j.ejc.2011.09.031}}.

\bibitem{DBLP:journals/dam/HochstattlerHMP21}
Winfried Hochst{\"{a}}ttler, Johann~L. Hurink, Bodo Manthey, Dani{\"{e}}l
  Paulusma, Britta Peis, and Georg Still.
\newblock In memoriam walter kern.
\newblock {\em Discret. Appl. Math.}, 303:2--3, 2021.
\newblock \href {https://doi.org/10.1016/j.dam.2021.08.034}
  {\path{doi:10.1016/j.dam.2021.08.034}}.

\bibitem{DBLP:journals/algorithmica/IoannidouMN11}
Kyriaki Ioannidou, George~B. Mertzios, and Stavros~D. Nikolopoulos.
\newblock The longest path problem has a polynomial solution on interval
  graphs.
\newblock {\em Algorithmica}, 61(2):320--341, 2011.
\newblock \href {https://doi.org/10.1007/s00453-010-9411-3}
  {\path{doi:10.1007/s00453-010-9411-3}}.

\bibitem{DBLP:journals/ipl/Keil85}
J.~Mark Keil.
\newblock Finding hamiltonian circuits in interval graphs.
\newblock {\em Inf. Process. Lett.}, 20(4):201--206, 1985.

\bibitem{DBLP:journals/algorithmica/KonstantinidisP21}
Athanasios~L. Konstantinidis and Charis Papadopoulos.
\newblock Cluster deletion on interval graphs and split related graphs.
\newblock {\em Algorithmica}, 83(7):2018--2046, 2021.
\newblock \href {https://doi.org/10.1007/s00453-021-00817-8}
  {\path{doi:10.1007/s00453-021-00817-8}}.

\bibitem{DBLP:journals/iandc/Kratsch87}
Dieter Kratsch.
\newblock Finding the minimum bandwidth of an interval graphs.
\newblock {\em Inf. Comput.}, 74(2):140--158, 1987.
\newblock \href {https://doi.org/10.1016/0890-5401(87)90028-9}
  {\path{doi:10.1016/0890-5401(87)90028-9}}.

\bibitem{DBLP:journals/siamdm/KratschS02}
Dieter Kratsch and Lorna Stewart.
\newblock Approximating bandwidth by mixing layouts of interval graphs.
\newblock {\em {SIAM} J. Discret. Math.}, 15(4):435--449, 2002.
\newblock \href {https://doi.org/10.1137/S0895480199359624}
  {\path{doi:10.1137/S0895480199359624}}.

\bibitem{lekkeikerker1962}
C.~Lekkeikerker and J.~Boland.
\newblock Representation of a finite graph by a set of intervals on the real
  line.
\newblock {\em Fundamenta Mathematicae}, 51(1):45--64, 1962.
\newblock URL: \url{http://eudml.org/doc/213681}.

\bibitem{DBLP:journals/dmgt/LinMW98}
In{-}Jen Lin, Terry~A. McKee, and Douglas~B. West.
\newblock The leafage of a chordal graph.
\newblock {\em Discuss. Math. Graph Theory}, 18(1):23--48, 1998.
\newblock \href {https://doi.org/10.7151/dmgt.1061}
  {\path{doi:10.7151/dmgt.1061}}.

\bibitem{DBLP:journals/jacm/LuekerB79}
George~S. Lueker and Kellogg~S. Booth.
\newblock A linear time algorithm for deciding interval graph isomorphism.
\newblock {\em J. {ACM}}, 26(2):183--195, 1979.

\bibitem{DBLP:journals/tcs/Marx06}
D{\'{a}}niel Marx.
\newblock Parameterized graph separation problems.
\newblock {\em Theor. Comput. Sci.}, 351(3):394--406, 2006.
\newblock \href {https://doi.org/10.1016/j.tcs.2005.10.007}
  {\path{doi:10.1016/j.tcs.2005.10.007}}.

\bibitem{DBLP:journals/siamcomp/MarxR14}
D{\'{a}}niel Marx and Igor Razgon.
\newblock Fixed-parameter tractability of multicut parameterized by the size of
  the cutset.
\newblock {\em {SIAM} J. Comput.}, 43(2):355--388, 2014.
\newblock \href {https://doi.org/10.1137/110855247}
  {\path{doi:10.1137/110855247}}.

\bibitem{DBLP:conf/mfcs/MisraP00S20}
Pranabendu Misra, Fahad Panolan, Ashutosh Rai, Saket Saurabh, and Roohani
  Sharma.
\newblock Quick separation in chordal and split graphs.
\newblock In Javier Esparza and Daniel Kr{\'{a}}l', editors, {\em 45th
  International Symposium on Mathematical Foundations of Computer Science,
  {MFCS} 2020, August 24-28, 2020, Prague, Czech Republic}, volume 170 of {\em
  LIPIcs}, pages 70:1--70:14. Schloss Dagstuhl - Leibniz-Zentrum f{\"{u}}r
  Informatik, 2020.
\newblock \href {https://doi.org/10.4230/LIPIcs.MFCS.2020.70}
  {\path{doi:10.4230/LIPIcs.MFCS.2020.70}}.

\bibitem{DBLP:journals/dam/Papadopoulos12}
Charis Papadopoulos.
\newblock Restricted vertex multicut on permutation graphs.
\newblock {\em Discret. Appl. Math.}, 160(12):1791--1797, 2012.
\newblock \href {https://doi.org/10.1016/j.dam.2012.03.021}
  {\path{doi:10.1016/j.dam.2012.03.021}}.

\bibitem{DBLP:journals/dam/PapadopoulosT19}
Charis Papadopoulos and Spyridon Tzimas.
\newblock Polynomial-time algorithms for the subset feedback vertex set problem
  on interval graphs and permutation graphs.
\newblock {\em Discret. Appl. Math.}, 258:204--221, 2019.
\newblock \href {https://doi.org/10.1016/j.dam.2018.11.017}
  {\path{doi:10.1016/j.dam.2018.11.017}}.

\bibitem{DBLP:conf/iwoca/PapadopoulosT22}
Charis Papadopoulos and Spyridon Tzimas.
\newblock Computing a minimum subset feedback vertex set on chordal graphs
  parameterized by leafage.
\newblock In Cristina Bazgan and Henning Fernau, editors, {\em Combinatorial
  Algorithms - 33rd International Workshop, {IWOCA} 2022, Trier, Germany, June
  7-9, 2022, Proceedings}, volume 13270 of {\em Lecture Notes in Computer
  Science}, pages 466--479. Springer, 2022.
\newblock \href {https://doi.org/10.1007/978-3-031-06678-8\_34}
  {\path{doi:10.1007/978-3-031-06678-8\_34}}.

\bibitem{walter1972representations}
James~Richard Walter.
\newblock {\em Representations of rigid cycle graphs}.
\newblock Wayne State University, 1972.

\bibitem{DBLP:journals/networks/WhiteFP85}
Kevin White, Martin Farber, and William~R. Pulleyblank.
\newblock Steiner trees, connected domination and strongly chordal graphs.
\newblock {\em Networks}, 15(1):109--124, 1985.
\newblock \href {https://doi.org/10.1002/net.3230150109}
  {\path{doi:10.1002/net.3230150109}}.

\end{thebibliography}

